Directions in Orbits of Geometrically Finite Hyperbolic Subgroups

We prove a theorem describing the limiting fine-scale statistics of orbits of a point in hyperbolic space under the action of a discrete subgroup. Similar results have been proved only in the lattice case, with two recent infinite-volume exceptions by Zhang for Apollonian circle packings and certain Schottky groups. Our results hold for general Zariski dense, non-elementary, geometrically finite subgroups in any dimension. Unlike in the lattice case, orbits of geometrically finite subgroups do not necessarily equidistribute on the whole boundary of hyperbolic space. But rather, they may equidistribute on a fractal subset. Understanding the behaviour of these orbits near the boundary is central to Patterson-Sullivan theory and much further work. Our theorem characterizes the higher order spatial statistics and thus addresses a very natural question. As a motivating example our work applies to sphere packings (in any dimension) which are invariant under the action of such discrete subgroups. At the end of the paper we show how this statistical characterization can be used to prove convergence of moments and to write down the limiting formula for the two-point correlation function and nearest neighbor distribution. Moreover we establish an formula for the 2 dimensional limiting gap distribution (and cumulative gap distribution) which was not known previously even in the lattice case.

==> Chapters/Equidistribution.tex <==
\section{Hyperbolic Geometry and Equidistribution Theorems}



\subsection{Infinite Volume Hyperbolic Spaces}

We now give a 'crash-course' introduction to measure theory on infinite volume hyperbolic surfaces. For a more in depth introduction we recommend the opening sections of the work by Oh and Shah \cite{OhShah2013} or the book by Borthwick \cite{Borthwick2007}


Throughout the presentation we adopt the following notation for subsets of $G$, given the point $i\in \half^n$ and a vector $X_i \in T^1(\half^n)$ based at $i$:

\begin{itemize}
  \item $A=\{a_t: t \in \R\}$ - a one-parameter subgroup of $G$, such that $r \mapsto (X)a_r$ is a unit speed geodesic flow for any $X \in T^1(\half^n)$
  \item $K := \SO(2)$, (note $K = \transpose{K}$) therefore $\operatorname{Stab}_G(i) = K$ and $\half^n \cong K\backslash G$.
  \item $M:= \mbox{Stab}_{G}(i)$, hence $G/M \cong T^{1}(\half^n)$
  \item $N^+ := \left\{ n \in G: \lim_{t\to \infty} a_t n a_{-t} = I \right\}$ - the expanding horocycle subgroup (corresponds to lower triangular matrices in 2D).
  \item $N^- := \left\{ n \in G: \lim_{t\to \infty} a_t n a_{-t} = I \right\}$ -  contracting horocycle subgroup (upper triangular matrices in 2D).
\end{itemize}

For $u \in T^1(\half^n)$ let 
\begin{equation}
  u^{\pm} = \lim_{t \to \pm \infty} (u)a_t.
\end{equation}
Let $\delta_{\Gamma}$ denote the \emph{critical exponent of the subgroup} $\Gamma$. Thus, $\delta_{\Gamma}$ is defined, for arbitrary $x,y \in \half^n$:

\begin{equation}
  \delta_{\Gamma} := \inf \{ s >0: \sum_{\gamma \in \Gamma} e^{-s d((x)\gamma,y)}<\infty \}.
\end{equation}
And let $\Lambda(\Gamma)$ denote the \emph{limit set of} $\Gamma$ (i.e the set of accumulation points of the orbit of (say) $i$). For the $\Gamma$ we are considering $\Lambda(\Gamma) \subset \partial \half^n$. 

For $\xi \in \partial \half^n$ and $x,y \in \half^n$ denote the \emph{Busemann function}, $\beta: \partial \half^n \times \half^n \times \half^n \to \R$:

\begin{equation}
  \beta_{\xi}(x,y) = \lim_{t \to \infty} d(x,\xi_t) - d(y, \xi_t)
\end{equation}
where $\xi_t $ is any geodesic ray such that as $\lim_{t\to \infty} \xi_t = \xi$ (the limiting value is independent of the choice of ray). In words $\beta_{\xi}(x,y)$ is the geodesic distance between two horospheres each based at $\xi$ containing $x$ and $y$ respectively.

With that, let $\{\mu_{x} : x \in \half^n\}$ denote a family of measures on $\partial \half^n$. We call such a family a \emph{$\Gamma$-invariant conformal density of dimension $\delta_{\mu} >0$} if: for each $x \in \half^n$, $\mu_x$ is a finite Borel measure and for all $y \in \half^n$, $\xi \in \partial \half^n$, and $\gamma \in \Gamma$:

\begin{eqnarray}
  \gamma_{\ast} \mu_x ( \cdot) := \mu_x(( \cdot )\gamma^{-1}) = \mu_{(x)\gamma}(\cdot)\\
  \frac{d\mu_x}{d\mu_y}(\xi) = e^{\delta_\mu \beta_{\xi}(y,x)}.
\end{eqnarray}

Building on Patterson's work in dimension $2$ \cite{Patterson1976}, Sullivan \cite{Sullivan1979}, by placing weighted delta measures on the orbit of $\Gamma$, proved the existence of a $\Gamma$-invariant conformal density of dimension $\delta_{\Gamma}$ supported on $\Lambda(\Gamma)$ which we will denote $\{\nu_x : x \in \half^n\}$ - the \emph{Patterson-Sullivan density}. 

Moreover let the \emph{Lesbegue density}, $\{m_{x} : x \in \half^n\}$ denote the $G$-invariant conformal density of dimension $(n-1)$, unique up to homothety. 

From here we can define several measures on $T^{1}(\half^n)$ which will be essential to what follows. For $u \in T^{1}(\half^n)$, let $\pi(u)$ be the projection to $\half^n$, $s:= \beta_{u^-}(i,\pi(u))$ and define:

\begin{itemize}
  \item The \emph{Bowen-Margulis-Sullivan} measure, given by:
    \begin{equation}
      dm^{BMS}(u) = e^{\delta_{\Gamma}\beta_{u^+}(i,\pi(u))}e^{\delta_{\Gamma}\beta_{u^-}(i,\pi(u))}d\nu_i(u^+)d\nu_i(u^-)ds.
    \end{equation}
    This measure is supported on $\{u \in T^{1}(\half^n) : u^+,u^- \in \Lambda(\Gamma)\}$ and is finite for geometrically finite $\Gamma$
  \item The \emph{Burger-Roblin} measure:
    \begin{equation}
      dm^{BR}(u) = e^{\delta_{\Gamma}\beta_{u^-}(i,\pi(u))}e^{(n-1)\beta_{u^+}(i,\pi(u))}d\nu_i(u^-)dm_i(u^+)ds.
    \end{equation}
    This measure is supported on $\{u \in T^{1}(\half^n) : u^- \in \Lambda(\Gamma)\}$


\end{itemize}

These are all measures on $T^{1}(\half^n) \cong G/M$. We extend them to measures on $G$. Consider for example the Burger-Roblin measure, for $\phi \in \mathcal{C}_{c}(G)$

\begin{equation}
  \int_{G} \phi (g) dm^{BR}(g) = \int_{T^1(\half^n)} \int_{M} \phi((u)m) dm dm^{BR}(u)
\end{equation}
where $dm$ is the normalized probability Haar measure on $M$. Thus we simply average out the extra dependence. To avoid too much notation we will use the same notation for both the measures on $G$ and $T^1(\half^n)$ as the definition will be clear.

Furthermore, given a horospherical subgroup $H < G$, let $\overline{H}:= H/M$ and define for $g \in G$

\begin{equation}
  d\tilde{\mu}_{g\overline{H}}^{PS}(gh):= e^{\delta_{\Gamma}\beta_{(gh)^-}(i,gh)} d\nu_0((gh)^-).
\end{equation}
We then let $d\mu^{PS}_{gH}$ (a measure on $gH$) denote the $H \cap M$-invariant extension. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%--------------SUBSECTION: EQUIDISTRIBUTION-------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Equidistribution Theorems}


Our goal is to apply an equidistribution theorem from Mohammadi-Oh \cite{MohammadiOh2015}, stated below, in the same way Marklof and Vinogradov \cite{MarklofVinogradov2018 } use their Theorem 2. Let $H$ be horospherical subgroup. Let $dh$ be the $H$-invariant Haar measure on $H$ and $d\overline{h}$ the $\overline{H}$-invariant Haar measure on $\overline{H}$ amd $d_{H \cap M}m$ the Haar measure normalized to be a probability measure on $H \cap M$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%---------------------------THEOREM - MOHAMMADI-OH------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem} {\cite[Theorem 5.3]{MohammadiOh2015}}   \label{thm:Mohammadi-Oh}
  For any $g \in G$, any $\Psi \in \mathcal{C}_c^{\infty}(\Gamma\backslash G)$ and $\phi \in \mathcal{C}_c^{\infty}(H)$, invariant under right multipication by $H \cap M$

  \begin{multline}\label{eqn: MO15 equi}
    \lim_{t \to \infty} e^{(n-1-\delta)t} \int_{\overline{H}}\int_{H \cap M} \Psi(\Gamma g \overline{h}m a_t) \phi(g\overline{h}) d\overline{h}d_{H \cap M}m\\  = \frac{1}{|m^{\operatorname{BMS}}|}\int_{\Gamma \backslash G \times (\Gamma \cap \overline{H})\backslash \overline{H}}\Psi(\alpha) \phi(g\overline{h})dm^{BR}(\alpha)d\mu_{\Gamma g\overline{H}}^{PS}(g\overline{h})
  \end{multline}

\end{theorem}
Note that the Theorem as stated by Mohammadi and Oh\cite{MohammadiOh15} does not require $\phi$ to be right $M$-invariant but for convenience of notation we make that assumption.

Let '$\operatorname{hor}$' denote a bijective parameterization of $g\overline{H}$ by $\R^{n-1}$. Thus $g\overline{H} =\{\operatorname{hor}(\vect{x}): \vect{x} \in \R^{n-1}\}$. We then let $\mu_{\hor}(\vect{x}): = d\mu_{\overline{H}}^{Haar}(\hor(\vect{x}))$ be the pull-back of the Haar measure on $g\overline{H}$ by $\hor$. And given a Borel probability measure $\lambda$ on $\R^{n-1}$ absolutely continuous with respect to Lesbegue we define $\lambda'(\vect{x}) := \frac{d\lambda}{d\mu_{\hor}}(\vect{x})$, the Radon-Nykodym derivative of $\lambda$. In that case we can then replace \prettyref{thm:Mohammadi-Oh} with the following corollary:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%------------------------COROLLARY: PROB-DENSITY--------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{corollary} \label{cor:prob-density}
  Under the assumptions of \prettyref{thm:Mohammadi-Oh}, let $\lambda$ be a compactly supported Borel probability measure on $\R^{n-1}$ with bounded and continuous, density, hence $\lambda' \in \mathcal{C}_c^{\infty}(\R^{n-1})$. Then for any $g \in G$

  \begin{multline}
    \lim_{t\to \infty} e^{(n-1-\delta)t}\int_{\R^{n-1}}\int_{M\cap \overline{H}} \Psi(\Gamma \hor (\vect{x})m a_t) d \lambda(\vect{x})d_{H \cap M}m \\= \frac{1}{|m^{BMS}|}\int_{\Gamma \backslash G \times (\Gamma \cap \overline{H}) \backslash \overline{H}}\lambda'(\hor^{-1}(g\overline{h}))\Psi(\alpha)dm^{BR}(\alpha)d\mu_{\Gamma g \overline{H}}^{PS}(g\overline{h})
  \end{multline}
\end{corollary}
 
From here, the proof of {\cite[Theorem 5.3]{MarklofStrom2010}} allows us to extend to functions of $\R^{d-1} \times \Gamma \backslash G$ and to sequences of functions

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-----------------------THEOREM: MULTIPLE FUNCTIONS-----------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{theorem} \label{thm:multiple-functions}
  Let $\lambda$ be as in Corollary \prettyref{cor:prob-density}. Let $f: \R^{n-1} \times \Gamma \backslash G \to \R$ be compactly supported, bounded and continuous. Let $f_t: \R^{n-1} \times \Gamma \backslash G \to \R$ be a uniformly bounded, compactly supported family of functions such that $f_t \to f$ uniformly. Then for any $g \in G$:  
  \begin{multline}
    \lim_{t\to \infty} e^{(n-1-\delta)t} \int_{\R^{n-1}\times M\cap \overline{H}} f_t(\vect{x}, \Gamma \hor(\vect{x})m a_t) d\lambda(\vect{x})d_{H\cap M}m\\ = \frac{1}{|m^{\operatorname{BMS}}|} \int_{\Gamma \backslash G \times (\Gamma\cap \overline{H}) \backslash \overline{H}}\lambda'(\hor^{-1}(g\overline{h})) f(\hor^{-1}(g\overline{h}), \alpha) dm^{BR}(\alpha)d\mu_{\Gamma g \overline{H}}^{PS}(g\overline{h})
  \end{multline}
\end{theorem}


\begin{proof}

  As $f_t$ converges to $f$ uniformly and all functions are uniformly continuous, for all $\delta>0$ there exist $\epsilon>0$ and $t_0>0$ such that

  \begin{equation}
    f(\vect{x}_0,g)-\delta \le f(\vect{x},g) , \; f_t(\vect{x},g) \le f(\vect{x}_0,g)+\delta
  \end{equation}
  for all $\vect{x} \in \vect{x}_0 + [0,\epsilon)^{n-1}$ and $t>t_0$. Furthermore

  \begin{multline}
    \int_{H\cap M}\int_{\R^{n-1}}f_t(\vect{x},\Gamma \hor(\vect{x})ma_t) d\lambda(\vect{x})d_{H\cap M}m \\
    = \sum_{\vect{k} \in \Z^{n-1}}\int_{H\cap M}\int_{\epsilon \vect{k}+[0,\epsilon)^{n-1}} f_t(\vect{x},\Gamma \hor(\vect{x})m a_t) d\lambda(\vect{x})d_{H\cap M}m\\
    \le  \sum_{\vect{k} \in \Z^{n-1}} \int_{H\cap M}\int_{\epsilon \vect{k}+[0,\epsilon)^{n-1}} f(\vect{x},\Gamma \hor(\vect{x})m a_t) d\lambda(\vect{x})d_{H\cap M}m+\delta
  \end{multline}
  Moreover, using Corollary \prettyref{cor:prob-density},

  \begin{align}
    &\lim_{t\to \infty} e^{(n-1-\delta)t} \int_{H\cap M}\int_{\epsilon \vect{k} + [0,\epsilon)^{n-1}} f(\vect{x},\Gamma \hor(\vect{x}) ma_t) d\lambda(\vect{x})d_{H\cap M}m\\ 
    &= \frac{1}{|m^{BMS}|} \int_{\Gamma\backslash G \times \Gamma \cap \overline{H} \backslash \overline{H}}\lambda'(\hor^{-1}(g\overline{h})) f(\epsilon \vect{k},\alpha)\mathbbm{1}_{\epsilon \vect{k}+[0,\epsilon)^{n-1}}(\hor^{-1}(g\overline{h})) dm^{BR}(\alpha)d\mu^{PS}_{\Gamma g\overline{H}}(g\overline{h})\\ 
    &= \frac{1}{|m^{BMS}|} \int_{\Gamma\backslash G \times \Gamma \cap \overline{H} \backslash \overline{H}}\lambda'(\hor^{-1}(g\overline{h})) (f(\hor^{-1}(g\overline{h}),\alpha)+\delta \mathbbm{1}_{\mbox{supp}(f(\hor^{-1}(g\overline{h}),\cdot))}(\alpha))\notag \\ 
    &\;\;\;\;\cdot \mathbbm{1}_{\epsilon \vect{k}+[0,\epsilon)^{n-1}}(\hor^{-1}(g\overline{h})) dm^{BR}(\alpha)d\mu^{PS}_{\Gamma g\overline{H}}(g\overline{h})\\
    &= \frac{1}{|m^{BMS}|} \int_{\Gamma\backslash G \times \Gamma \cap \overline{H} \backslash \overline{H}}\lambda'(\hor^{-1}(g\overline{h})) f(\hor^{-1}(g\overline{h}),\alpha)\mathbbm{1}_{\epsilon \vect{k}+[0,\epsilon)^{n-1}}(\hor^{-1}(g\overline{h})) dm^{BR}(\alpha)d\mu^{PS}_{\Gamma g\overline{H}}(g\overline{h}) \notag\\
    &\;\;\;\;+ C \delta
  \end{align}
  Putting this all together we get, for any $\delta$:

  \begin{multline}
    \limsup_{t\to \infty} e^{(n-1-\delta)t} \int_{\R^{n-1}\times H \cap M} f_t(\vect{x}, \Gamma \hor(\vect{x})m a_t) d\lambda(\vect{x})d_{H\cap M}m \\\le \frac{1}{|m^{\operatorname{BMS}}|} \int_{\Gamma \backslash G  \times \Gamma\cap \overline{H} \backslash \overline{H}} \lambda'(\hor^{-1}(g\overline{h}))f(\hor^{-1}(g\overline{h}), \alpha)dm^{BR}(\alpha) d\mu^{PS}_{\Gamma g\overline{H}}(g\overline{h}) +C\delta.
  \end{multline}
  A similar bound can be achieved for the $\liminf$ from which the Theorem follows.

\end{proof}



% Now let $\{ \mathcal{E}_t\}_{t\ge t_0}$ be bounded subsets of $\R^{n-1} \times \Gamma \backslash G$ all with $0$ boundary when measured with the $\lambda \times m^{BR}$ for some fixed $t_0>0$ and define:

% \begin{eqnarray}
%   \lim \left( \inf \mathcal{E}_t \right)^o &:=& \bigcup_{t \ge t_0} \left( \bigcap_{s \ge t} \mathcal{E}_s \right)^o \\
%   \lim \overline{ \sup \mathcal{E}_t} &:=& \bigcap_{t \ge t_0} \overline{ \bigcup_{s \ge t} \mathcal{E}_s }
% \end{eqnarray}


% In which case we arrive at the same Corollary as [\cite{MarklofStrom2010} - Theorem 5.6]:


 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %-------------------------COROLLARY - TEST-FUNCTIONS----------------------------
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \begin{corollary}\label{cor:test-functions}
%   Let $\lambda$ be a Borel probability measure on $\R^{n-1}$ as in Corollary \prettyref{cor:prob-density}. Then for any family of subsets $\mathcal{E}_t \subset \R^{n-1} \times \Gamma \backslash G$ such that $\lambda \times m^{BR}(\partial (\lim (\overline{ \sup \mathcal{E}_t}))) = \lambda \times m^{BR}(\partial( \lim  (\inf \mathcal{E}_t)^o))  = 0$ we have for any $g \in \Gamma \backslash G$:

%   \begin{multline}
%      \liminf_{t \to \infty} e^{(n-1-\delta)t} \int_{\R^{n-1}}\chi_{\mathcal{E}_t} (\vect{x}, g n(\vect{x}) a_t) d\lambda(\vect{x}) \ge A_{\lambda} \int_{\lim(\inf\mathcal{E}_t)^o} d\lambda(\vect{x}) dm^{BR}(h) 
%   \end{multline}
%   \begin{multline}
%     \limsup_{t \to \infty} e^{(n-1-\delta)t} \int_{\R^{n-1}}\chi_{\mathcal{E}_t} (\vect{x}, g n(\vect{x}) a_t) d\lambda(\vect{x}) \le A_{\lambda} \int_{\lim\overline{\sup\mathcal{E}_t}} d\lambda(\vect{x}) dm^{BR}(h) \label{eqn:limsup}
%   \end{multline}
%   Moreover, if $\lambda \times m^{BR}$ gives zero measure to $\lim\overline{\sup\mathcal{E}_t} \setminus \lim(\inf\mathcal{E}_t)^o$ then:

%   \begin{equation}
%     \lim_{t \to \infty} e^{(n-1-\delta)t} \int_{\R^{n-1}}\chi_{\mathcal{E}_t} (\vect{x}, g n(\vect{x}) a_t) d\lambda(\vect{x})  =  A_{\lambda} \int_{\lim\sup\mathcal{E}_t} d\lambda(\vect{x}) dm^{BR}(h) 
%   \end{equation}
% \end{corollary}

% \begin{proof}

%   This Corollary follows from \prettyref{thm:multiple-functions} in exactly the same way as Theorem 5.6 follows in \cite{MarklofStrom2010}, with the one exception. Addressing only (\ref{eqn:limsup}) (as the other results follow similarly). Let:

%   \begin{equation}
%     \tilde{\mathcal{E}}_t := \overline{\bigcup_{s \ge t}\mathcal{E}_s}
%   \end{equation}
%   this is a closed set and the proof of [\cite{MarklofStrom2010} Theorem 5.6] involves using the analogue of \prettyref{thm:multiple-functions} by approximating $\chi_{\tilde{\mathcal{E}}_t}$ by bounded continuous functions. This arguement follows exactly as in the proof of the extension of \prettyref{thm:Mohammadi-Oh} to piecewise continuous functions and is the reason why we need to have the boundaries of measure $0$ (although now we are using the $BR$-measure).


% \end{proof}



==> Chapters/_region_.tex <==
\message{ !name(5_Cuspidal_Moments.tex)}
\message{ !name(5_Cuspidal_Moments.tex) !offset(-2) }
\section{Moment Generating Function for Cuspidal Observer}

Continuing to follow the example set by \cite{MarklofVinogradov2018}, for test sets $\mathcal{A}_1,..., \mathcal{A}_m \subset \R^{n-1}$ with boundary of Lesbesgue measure $0$ and for complex $\tau_i \in \C$, define the moment generating function

\begin{equation}
  \mathbb{G}_{t,s}^{\infty}(\tau_1,...,\tau_m; \mathcal{A}) := \int_{\T^l \times \R^{n-1-l}} \mathbbm{1}(\mathcal{N}_{t,s}^{\infty}(\mathcal{A}_j,\vect{x}, \overline{\vect{w}}) \neq 0, \forall j)\exp\left(\sum_{j=1}^m \tau_j \mathcal{N}_{t,s}^{\infty}(\mathcal{A}_j,\vect{x}, \overline{\vect{w}})   \right) d\lambda(\vect{x})
\end{equation}
and similarly for the limit distribution let

\begin{equation}
  \mathbb{G}_{s}(\tau_1,...,\tau_m; \mathcal{A}) := \sum_{r_1,...,r_m=1}^{\infty} \exp \left(\sum_{j=1}^m \tau_j r_j  \right)E_s(r,\mathcal{A},\overline{\vect{w}}).
\end{equation}
Where $E_s$ is defined as in \prettyref{thm:joint-limit} and $r=(r_1,...,r_m)$. Let $\operatorname{Re}_+ \tau := \max (\operatorname{Re}(\tau),0)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%----------------THEOREM: MOMENT-GENERATING-------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{theorem} \label{thm:moment-generating}
  Let $\lambda$ be a Borel probability measure on $\T^l \times \R^{n-1-l}$ as in \prettyref{thm:joint-limit}, and $\{\mathcal{A}\}_{j=1}^m \subset \R^{(n-1)}$ bounded with boundary of Lesbegue measure $0$. Then there exists a constant $c_0>0$ such that for $\operatorname{Re}_+ \tau_1 + ... + \operatorname{Re}_+\tau_m < c_0$, $s \in (0,\infty]$

  \begin{enumerate}
    \item $\mathbb{G}_s(\tau_1,..., \tau_m;\mathcal{A})$ is analytic
    \item $\lim_{t\to \infty}e^{(n-1-\delta_{\Gamma})t} \mathbb{G}_{t,s}^{\infty}(\tau_1,..., \tau_m;\mathcal{A})= \frac{A_{\lambda}}{|\mathrm{m}^{BMS}|}\mathbb{G}_s(\tau_1,..., \tau_m;\mathcal{A})$.
  \end{enumerate}

\end{theorem}



Suppose $-\infty < a< b \le \infty$ and $\mathcal{A} \subset \R^{n-1}$
 
\begin{equation}
  \mathcal{Z}(a,b,\mathcal{A}):= \{ \vect{z} \in \half^n : \operatorname{Re}\vect{z} \in \vartheta^{-1/\delta_{\Gamma}}\mathcal{A}, e^a \le \operatorname{Im} \vect{z} \le e^b \}
\end{equation}
For $b<\infty$ this quanitity is bounded, and thus $\#(\overline{\vect{w}}g \cap \mathcal{Z}(a,b,\mathcal{A}))$ is bounded from above uniformly in $g$. This implies that all moments converge. Therefore we are concerned with the case $b=\infty$.

For that, let 

\begin{equation}
  \delta(\overline{\vect{w}}g):= \min_{\substack{\gamma_1,\gamma_2 \in \Gamma\\  \gamma_1 \not\in \Gamma_w\gamma_2}} d(\vect{w}\gamma_1g, \vect{w}\gamma_2g).
\end{equation}
Note, because $g$ is an isometry and because $G$ acts properly dicontinuously

\begin{equation}
  \delta(\overline{\vect{w}}g) = \min_{\gamma \in \Gamma_{\vect{w}} \backslash \Gamma} d(\vect{w},\vect{w}\gamma )=\delta(\overline{\vect{w}})>0.
\end{equation}





In order to prove \prettyref{thm:moment-generating} we first require three lemmas (as is the case in \cite{MarklofVinogradov2018}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%---------------------------LEMMA: MV-LEMMA-10----------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma} \label{lem:MV-Lemma-10}
  Fix $a\in \R$ and a bounded subset $\mathcal{A} \subset \R^{n-1}$. There exist positive constant $\zeta, \eta$ such that for all $g \in G$, $r\in \N$

  \begin{equation}
    \left[ \#(\overline{\vect{w}}g \cap \mathcal{Z}(a,\infty, \mathcal{A}))\ge r \right ] \Rightarrow \left[ \#(\overline{\vect{w}}g \cap \mathcal{Z}(\zeta r - \eta,\infty, \mathcal{A}))\ge 1 \right]
  \end{equation}

\end{lemma}

This lemma is a statement about the definition of $\mathcal{Z}$. As the definition is the same as \cite{MarklofVinogradov2018} we do not include the proof (see {\cite[Lemma 10]{MarklofVinogradov2018}})






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%------------------------------LEMMA: MV-Lemma 11-------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{lem:MV-Lemma-11}
  Fix a bounded subset $\mathcal{A} \subset \R^{n-1}$ and $\zeta, \eta $ as in \prettyref{lem:MV-Lemma-10}. Then

  \begin{eqnarray}
    \int_{\Gamma \backslash G} \# (\overline{\vect{w}}g \cap \mathcal{Z}(\zeta r - \eta, \infty,\mathcal{A}))d\mathrm{m}^{BR}(g) \le  \frac{e^{(-\delta_{\Gamma^w}-n+1)(\zeta r - \eta)}\vartheta^{(n-1)/\delta_{\Gamma}}\vol_{\half^n}(\mathcal{A})}{\#\Gamma_{\vect{w}}(n-1)}
  \end{eqnarray}

\end{lemma}


\begin{proof}
  
  This statement follows quite straightfowardly from Proposition \prettyref{prop:MV-Lemma-5} and specifically (\ref{eqn:thin-Siegel}). To see this note

  \begin{eqnarray}
    &&\int_{\Gamma \backslash G} \# (\overline{\vect{w}}g \cap \mathcal{Z}(\zeta r - \eta, \infty,\mathcal{A}))d\mathrm{m}^{BR}(g)\label{eqn:LM11-eqn1}\\
    &=& \frac{1}{\#\Gamma_{\vect{w}}} \int_G \chi_{\mathcal{Z}(\zeta r-\eta , \infty, \mathcal{A})}( \vect{w}g) d\mathrm{m}^{BR}(g) \label{eqn:LM11-eqn2}\\
    &\le& \frac{e^{-\delta_{\Gamma^{\vect{w}}(\zeta r - \eta)}}}{\#\Gamma_{\vect{w}}}\vol_{\half^n}(g^{-1}_{\vect{w}} \mathcal{Z}(\zeta r - \eta, \infty, \mathcal{A})) \label{eqn:LM11-eqn3}\\
    &=& \frac{e^{(-\delta_{\Gamma^{\vect{w}}}-n+1)(\zeta r - \eta)}\vartheta^{(n-1)/\delta_{\Gamma}}\vol_{\half^n}(\mathcal{A})}{\#\Gamma_{\vect{w}}(n-1)} \label{eqn:LM11-eqn4}.
  \end{eqnarray}


\end{proof}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%-------------------------LEMMA: MV-Lemma-12------------------------------------
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{lem:MV-Lemma-12}
  Fix a bounded subset $\mathcal{A} \subset \R^{n-1}$ and $\zeta,\eta$ as in \prettyref{lem:MV-Lemma-10}. Let $\lambda$ be a probability measure on $\T^l \times \R^{n-1-l}$ as in \prettyref{thm:joint-limit}. Then, there exists a constant $C$ such that

  \begin{equation}
    \sup_{t \ge 0}\int_{\T^l \times \R^{n-1-l}} \# (\overline{\vect{w}}n(\vect{x})a_t \cap \mathcal{Z}(\zeta r - \eta, \infty, \mathcal{A})) d \lambda(\vect{x}) \le Ce^{-\zeta r \delta_{\Gamma}}.
   \end{equation}
\end{lemma}

\begin{proof}

  The proof follows very similar lines to {\cite[Lemma 12]{MarklofVinogradov2018}}. Firstly by taking $C$ large we may assume $\lambda$ is the Lesbegue measure. Then

  \begin{eqnarray}
    &&\int_{\T^l \times \R^{n-1-l}} \# (\overline{\vect{w}}n(\vect{x})a_t \cap \mathcal{Z}(\zeta r - \eta, \infty, \mathcal{A}))d\vect{x} \\ 
    &=& \int_{\T^l \times \R^{n-1-l}} \# (\overline{\vect{w}}n(\vect{x}) \cap \mathcal{Z}(\zeta r - \eta-t, \infty, e^{-t}\mathcal{A})) d\vect{x}\\
    &=& \vol_{\R^{n-1}}(e^{-t}\mathcal{A}) \# \{ \gamma \in \Gamma_{\vect{w}} \backslash \Gamma /\Gamma_\infty, \operatorname{Im}(\vect{w}\gamma) \ge e^{-t+\zeta r - \eta}\}.
  \end{eqnarray}
  By (\ref{eqn:P-asymptotics}) there exists a constant such that

  \begin{equation}
    \# \{ \gamma \in \Gamma_{\vect{w}} \backslash \Gamma /\Gamma_\infty, \operatorname{Im}(\vect{w}\gamma) \ge e^{-t+\zeta r - \eta}\} \le C' \max\{1,e^{-\delta_{\Gamma}(t-\zeta r)}\}.
  \end{equation}
  from which the Lemma follows.
 
\end{proof}



\begin{proof}[Proof of \prettyref{thm:moment-generating}]
  To begin with we once more note that for $s<\infty$, $\mathcal{N}_{t,s}^{\infty}(\mathcal{A}_j, \vect{x}; \overline{\vect{w}})$ is uniformly bounded and thus $E_s(r,\mathcal{A}; \overline{\vect{w}}) = 0$ for $|r|:=\max_j r_j$ large enough. From here the Theorem follows. Thus we set $s=\infty$ for the remainder of the proof.
  
  Set $\tilde{\mathcal{A}} = \bigcup_j \mathcal{A}_j$

  \begin{eqnarray}
    \sum_{|s| \ge R} E(r,\mathcal{A}; \overline{\vect{w}}) &\le& \sum_{r'=R}^{\infty}E_s(r',\tilde{\mathcal{A}}; \overline{\vect{w}})\\
                     &\le& \frac{A_{\lambda}}{|\mathrm{m}^{BMS}|}\mathrm{m}^{BR}(\{ g \in \Gamma \backslash G : \#(\overline{\vect{w}} g \cap \mathcal{Z}(0,\infty, \tilde{\mathcal{A}}) \ge R\}) \nonumber\\
                     &\le& \frac{A_{\lambda}}{|\mathrm{m}^{BMS}|} \mathrm{m}^{BR}(\{ g \in \Gamma \backslash G : \#(\overline{\vect{w}} g \cap \mathcal{Z}(\zeta R - \eta,\infty, \tilde{\mathcal{A}}) \ge 1\}) \nonumber\\
                     &\le& \frac{A_{\lambda}}{|\mathrm{m}^{BMS}|} \int_{\Gamma \backslash G} \# (\overline{\vect{w}}g \cap \mathcal{Z}( \zeta R - \eta, \infty, \tilde{\mathcal{A}})) d\mathrm{m}^{BR}(g).
  \end{eqnarray}
  where we have used \prettyref{lem:MV-Lemma-10} and Chebychev's inequality.

  We can then use \prettyref{lem:MV-Lemma-11} to say

  \begin{equation}
    \sum_{|r| \ge R} E_s(r,\mathcal{A};\overline{\vect{w}}) \le C_1 e^{-\delta_{\Gamma}\zeta R}
  \end{equation}
  from which analyticity follows. 

  \prettyref{thm:joint-limit} implies

  \begin{multline}
    \lim_{t\to \infty} e^{(n-1-\delta_{\Gamma})t}\int_{\T^l \times \R^{n-1-l}}\prod_{j=1}^m \mathbbm{1}(0<\mathcal{N}_{t,s}^{\infty}(\mathcal{A}_j,\vect{x};\overline{\vect{w}}) <R) \exp (\tau_j \mathcal{N}_{t,s}^{\infty}(\mathcal{A}_j,\vect{x}; \overline{\vect{w}}))d\lambda(\vect{x}) \\
    = \frac{A_{\lambda}}{|\mathrm{m}^{BMS}|}\sum_{r_1,...,r_m=1}^{R-1}\exp\left( \sum_{j=1}^m \tau_j r_j\right) E_s(r,\mathcal{A}; \overline{\vect{w}}).
  \end{multline}
  Therefore it remains to show
  
  \begin{multline}
    \lim_{R \to \infty}\limsup_{t\to \infty}\left| \int_{\T^l \times \R^{n-1-l}}\prod_{j=1}^m \mathbbm{1}(\max_j\mathcal{N}_{t,s}^{\infty}(\mathcal{A}_j,\vect{x};\overline{\vect{w}}) <R , \min_j\mathcal{N}_{t,s}^{\infty}(\mathcal{A}_j,\vect{x};\overline{\vect{w}}) >0 ) \exp (\tau_j \mathcal{N}_{t,s}^{\infty}(\mathcal{A}_j,\vect{x}; \overline{\vect{w}}))d\lambda(\vect{x})\right| =0
  \end{multline}
  Note that

  \begin{multline}
    \left| \int_{\T^l \times \R^{n-1-l}}\prod_{j=1}^m \mathbbm{1}(\max_j\mathcal{N}_{t,s}^{\infty}(\mathcal{A}_j,\vect{x};\overline{\vect{w}}) \ge R) \exp (\tau_j \mathcal{N}_{t,s}^{\infty}(\mathcal{A}_j,\vect{x}; \overline{\vect{w}}))d\lambda(\vect{x})\right| \\\le \int_{\T^l \times \R^{n-1-l}}\mathbbm{1}(\mathcal{N}_{t,s}^{\infty}(\mathcal{A},\vect{x}; \overline{\vect{w}}) \ge R)\exp (\tilde{\tau}\mathcal{N}_{t,s}^{\infty}(\tilde{\mathcal{A}},\vect{x};\overline{\vect{w}}))d\lambda(\vect{x}),
  \end{multline}
  where $\tilde{\mathcal{A}}= \bigcup_j \mathcal{A}_j$ and $\tilde{\tau} = \sum_j \operatorname{Re}_+\tau_j$. From there, performing the same decomposition as {\cite[proof of Theorem 8]{MarklofVinogradov2018}} we get that the above is less than

  \begin{equation}
    \le \sum_{r=R}^{\infty} e^{\tilde{\tau}r}\int_{\T^l \times \R^{n-1-l}}\mathbbm{1}(\mathcal{N}_{t,s}^{\infty}(\tilde{\mathcal{A}},\vect{x};\overline{\vect{w}})\ge r )d\lambda(\vect{x}).
  \end{equation}
  Which we can bound (uniformly in $t \ge 0$) using \prettyref{lem:MV-Lemma-10} and \prettyref{lem:MV-Lemma-12} by

  \begin{equation}
\le \sum_{r=R}^{\infty} C e^{\tilde{\tau}r}e^{-\delta_{\Gamma} \zeta r}.
  \end{equation}
  Thus, for $\tilde{\tau} < \delta_{\Gamma} \zeta$

  \begin{equation}
    \lim_{R \to 1} \sum_{r=R}^{\infty} e^{\tilde{\tau}r}\int_{\T^l \times \R^{n-1-l}}\mathbbm{1}(\mathcal{N}_{t,s}^{\infty}(\tilde{\mathcal{A}},\vect{x};\overline{\vect{w}})\ge r )d\lambda(\vect{x}) = 0
  \end{equation}
  uniformly in $t$. Taking $c_0=\delta_{\Gamma} \zeta$ proves the Theorem.


\end{proof}





\message{ !name(5_Cuspidal_Moments.tex) !offset(-208) }

